Provable Pathways: Learning Multiple Tasks over Multiple Paths

Constructing useful representations across a large number of tasks is a key requirement for sample-efficient intelligent systems. A traditional idea in multitask learning (MTL) is building a shared representation across tasks which can then be adapted to new tasks by tuning last layers. A desirable refinement of using a shared one-fits-all representation is to construct task-specific representations. To this end, recent PathNet/muNet architectures represent individual tasks as pathways within a larger supernet. The subnetworks induced by pathways can be viewed as task-specific representations that are composition of modules within supernet's computation graph. This work explores the pathways proposal from the lens of statistical learning: We first develop novel generalization bounds for empirical risk minimization problems learning multiple tasks over multiple paths (Multipath MTL). In conjunction, we formalize the benefits of resulting multipath representation when adapting to new downstream tasks. Our bounds are expressed in terms of Gaussian complexity, lead to tangible guarantees for the class of linear representations, and provide novel insights into the quality and benefits of a multipath representation. When computation graph is a tree, Multipath MTL hierarchically clusters the tasks and builds cluster-specific representations. We provide further discussion and experiments for hierarchical MTL and rigorously identify the conditions under which Multipath MTL is provably superior to traditional MTL approaches with shallow supernets.

==> app/proof_cluster.tex <==
\begin{proof}
    Let $\hat\phi,~\hat\A,~\hat\bho,~\hat\h$ be the empirical solution of (\ref{formula:cluster}) and $\phi^\star,~\A^\star,~\bho^\star,~\h^\star$ be the population solution of (\ref{formula:cluster}) when each task has infinite i.i.d training samples ($N=\infty$). Let $\Lc(\f)=\frac{1}{T}\sum_{t=1}^T\E_{\Dc_t}[\ell(h_t\circ\omega_{A(t)}\circ\phi(\x_t),y_t)]$ and $\hat\Lc(\f)=\frac{1}{NT}\sum_{t=1}^T\sum_{i=1}^N\ell(h_t\circ\omega_{A(t)}\circ\phi(\x_{t,i}),y_{t,i})$.
    % $\Lc(\f)=\E_{\bar{\Dc}}[\hat\Lc(\f)]$, where $\bar\Dc:=\frac{1}{T}\sum_{t=1}^T\Dc_t$. 
    Then we have
    \begin{align}
    \Lc(\hat \f)-\Lc(\f^\star)&=\underset{a}{\underbrace{\Lc(\hat \f)-\hat\Lc(\hat \f)}} + \underset{b}{\underbrace{\hat\Lc(\hat \f)-\hat\Lc(\f^\star)}} + \underset{c}{\underbrace{\hat\Lc(\f^\star)-\Lc(\f^\star)}},
    \end{align}
    where $b\leq0$ since of the fact that $\hat \f$ is the empirical risk minimizer of $\hat\Lc(\f)$. Define the search space of function $\f$ by $\Fc$. 
    %, then we have $a,c\leq\sup_{\f\in\Fc}|\Lc(\f)-\hat\Lc(\f)|$. 
    Rewrite samples in $\Dc_t$ as $(\x_i,y_i,t_i\equiv t)$. Then, we can define distribution $\bar\Dc=\frac{1}{T}\sum_{t=1}^T\Dc_t$ and the task identification-aware multitask training dataset can be seen as $\Sc=(\x_i,y_i,t_i)_{i=1}^{NT}\overset{\text{i.i.d.}}{\sim}\bar\Dc^{NT}$. The loss functions can be rewritten by $\Lc(\f)=\E_{\bar\Dc}[\ell(\f(\x,t),y)]$, $\hat\Lc(\f)=\frac{1}{NT}\sum_{i=1}^{NT}\ell(\f(\x_i,t_i),y_i)$ and $\Lc(\f)=\E_{\bar\Dc}[\hat\Lc(\f)]$, where $\f(\x,t)=f_t(\x)=h_t\circ\omega_{A(t)}\circ\phi(\x)$ and $t\in[T]$. 
    Then, following the Theorem~3.3 of \cite{mohri2018foundations}, we have that with probability at least $1-\frac{\delta}{2}$, $
    a\leq\sup_{\f\in\Fc}\Lc(\f)-\hat\Lc(\f)\leq2\Rc_{NT}(\ell(\Fc))+\sqrt{\frac{\log\frac{2}{\delta}}{2NT}}$.
    Next using the facts that the theorem still holds if we replace loss function with its negative and $\Rc(\ell(\Fc))=\Rc(-\ell(\Fc))$, we have that with probability at least $1-\frac{\delta}{2}$, $c\leq2\Rc_{NT}(\ell(\Fc))+\sqrt{\frac{\log\frac{2}{\delta}}{2NT}}$. Combining them, we can conclude that with probability at least $1-\delta$,
    \begin{align}
        \Lc(\hat \f)-\Lc(\f^\star)&\leq4\Rc_{NT}(\ell(\Fc))+\sqrt{\frac{2\log\frac{2}{\delta}}{NT}}, \\
        \text{and similarly,}~~~\Lc(\hat \f)-\Lc(\f^\star)&\leq4\hat\Rc_{\Sc}(\ell(\Fc))+3\sqrt{\frac{2\log\frac{4}{\delta}}{NT}},
    \end{align}
    where $\hat\Rc_{\Sc}(\ell(\Fc))$ is the empirical Rademacher complexity as follows.
    \begin{align}
        \hat\Rc_{\Sc}(\ell(\Fc))&:=\E_{\bsgm}\left[\sup_{\f\in\Fc}\frac{1}{NT}\sum_{i=1}^{NT}\sigma_{i}\ell(\f(\x_{i},t_i),y_{i})\right]\\
        &\leq\E_{\bsgm}\left[\sup_{\f\in\Fc}\frac{1}{NT}\sum_{i=1}^{NT}\sigma_{i}L|\f(\x_{i},t_i)-y_{i}|\right]\\
        &\leq\E_{\bsgm}\left[\sup_{\f\in\Fc}\frac{1}{NT}\sum_{i=1}^{NT}\sigma_{i}L|\f(\x_{i},t_i)|\right]+\underset{=0}{\underbrace{\E_{\bsgm}\left[\frac{1}{NT}\sum_{i=1}^{NT}\sigma_{i}L|y_{i}|\right]}} \\
        &\leq L\cdot\E_{\bsgm}\left[\sup_{\f\in\Fc}\frac{1}{NT}\sum_{i=1}^{NT}\sigma_{i}\f(\x_{i},t_i)+\E_{\bsgm}\sup_{\f\in\Fc}\frac{1}{NT}\sum_{i=1}^{NT}\sigma_{i}\cdot(-\f(\x_{i},t_i))\right] \\
        &=2L\cdot\E_{\bsgm}\left[\sup_{\f\in\Fc}\frac{1}{NT}\sum_{i=1}^{NT}\sigma_{i}\f(\x_{i},t_i)\right]=2L\hat\Rc_{\X}(\Fc),
        % \\
        % \Rc_{NT}(\ell(\Fc))&:=\underset{(\x_{i},y_{i},t_i)_{i=1}^{NT}\sim\bar\Dc^{NT}}{\E}\left[\E_{\bsgm}\sup_{\f\in\Fc}\frac{1}{NT}\sum_{i=1}^{NT}\sigma_{i}\ell(\f(\x_{i},t_i),y_{i})\right]\\
        % &\leq{\E}\left[\E_{\bsgm}\sup_{\f\in\Fc}\frac{1}{NT}\sum_{i=1}^{NT}\sigma_{i}L|\f(\x_{i},t_i)-y_{i}|\right]\\
        % &\leq{\E}\left[\E_{\bsgm}\sup_{\f\in\Fc}\frac{1}{NT}\sum_{i=1}^{NT}\sigma_{i}L|\f(\x_{i},t_i)|+\underset{=0}{\underbrace{\E_{\bsgm}\frac{1}{NT}\sum_{i=1}^{NT}\sigma_{i}L|y_{i}|}}\right] \\
        % &\leq L\cdot{\E}\left[\E_\bsgm\sup_{\f\in\Fc}\frac{1}{NT}\sum_{i=1}^{NT}\sigma_{i}\f(\x_{i},t_i)+\E_{\bsgm}\sup_{\f\in\Fc}\frac{1}{NT}\sum_{i=1}^{NT}\sigma_{i}\cdot(-\f(\x_{i},t_i))\right] \\
        % &=2L\cdot{\E}\left[\E_{\bsgm}\sup_{\f\in\Fc}\frac{1}{NT}\sum_{i=1}^{NT}\sigma_{i}\f(\x_{i},t_i)\right]=2L\Rc_{NT}(\Fc),
    \end{align}
    and $\Rc_{NT}(\ell(\Fc))=\E[\hat\Rc_\Sc(\ell(\Fc))]\leq2L\E[\hat\Rc_\X(\Fc)]$.
    
    
    % where $\Rc_{NT}$ is the Rademacher complexity of sample size $NT$ and distribution $\bar\Dc:=\frac{1}{T}\sum_{t=1}^T\Dc_{t}$. Now we need to decompose $\Rc_{NT}(\ell(\Fc))$. To ease the notation, we use $m=NT$ in the following.
    % \begin{align}
    %     \Rc_{m}(\ell(\Fc))&:=\underset{(\x_i,y_i)_{i=1}^m\sim\bar\Dc^m}{\E}\left[\E_{\sigma_i}\sup_{f\in\Fc}\frac{1}{m}\sum_{i=1}^m\sigma_i\ell(f(\x_i),y_i)\right]\\
    %     &\leq\underset{(\x_i,y_i)_{i=1}^m\sim\bar\Dc^m}{\E}\left[\E_{\sigma_i}\sup_{f\in\Fc}\frac{1}{m}\sum_{i=1}^m\sigma_iL|f(\x_i)-y_i|\right]\\
    %     &\leq \underset{(\x_i,y_i)_{i=1}^m\sim\bar\Dc^m}{\E}\left[\E_{\sigma_i}\sup_{f\in\Fc}\frac{1}{m}\sum_{i=1}^m\sigma_iL|f(\x_i)|+\underset{=0}{\underbrace{\E_{\sigma_i}\sup_{f\in\Fc}\frac{1}{m}\sum_{i=1}^m\sigma_iL|y_i|}}\right] \\
    %     &\leq L\underset{(\x_i,y_i)_{i=1}^m\sim\bar\Dc^m}{\E}\left[\E_{\sigma_i}\sup_{f\in\Fc}\frac{1}{m}\sum_{i=1}^m\sigma_if(\x_i)+\E_{\sigma_i}\sup_{f\in\Fc}\frac{1}{m}\sum_{i=1}^m\sigma_i\cdot(-f(\x_i))\right] \\
    %     &=2L\underset{(\x_i,y_i)_{i=1}^m\sim\bar\Dc^m}{\E}\left[\E_{\sigma_i}\sup_{f\in\Fc}\frac{1}{m}\sum_{i=1}^m\sigma_if(\x_i)\right]=2L\Rc_m(\Fc).
    % \end{align}
    Now, it remains to decompose the Rademacher complexity of a set of combination functions $\Fc$ over basic function sets $\Hc,~\Ac,~\Omega$ and $\Phi$.
    % Since $\omega_{A(t)}$ is not interpretable, we can write the prediction function as $f_t=h_t\circ\A_t\circ\bho\circ\phi$, where $\A_t\in\R^K$ is the $t_{\text{th}}$ row of the clustering matrix and it is an one-hot vector with the nonzero index $A(t)\in\{1,2\dots,K\}$. In a nutshell, we decompose $\omega_{A(t)}=\A_t\circ\bho$. Now we have $\Rc_{NT}(\Fc):=\Rc_{NT}(\Hc^T\circ\Ac\circ\Omega^K\circ\Phi)$ and it remains to decompose the Rademacher complexity of a set of combination functions $\Fc$ over basic function sets $\Hc,~\Ac,~\Omega$ and $\Phi$.
    
    Inspired by \cite{tripuraneni2020theory}, we use the Dudley's entropy integral bound showed in \cite{wainwright2019high} (Theorem~5.22) to derive the upper bound.  Define $Z_{\f}:=\frac{1}{\sqrt{NT}}\sum_{i=1}^{NT}\sigma_{i}\f(\x_{i},t_i)$ where $\f\in\Fc$ and $\sigma_{i}$ are Rademacher random variables uniformly taking values in $\{1, -1\}$. Hence, $Z_{\f}$ are zero-mean random Gaussian variables for any given $\f\in\Fc$. Given task ID-aware training inputs $\X=\{(\x_i,t_i):i\in[NT],t_i\in[T]\}$, we have $\hat\Rc_{\X}(\Fc)=\frac{1}{\sqrt{NT}}\E_{\bsgm}[\sup_{\f\in\Fc}Z_{\f}]\leq\frac{1}{\sqrt{NT}}\E_{\bsgm}[\sup_{\f,\f'\in\Fc}(Z_{\f}-Z_{\f'})]$. Define the distance of $\f,~\f'$ given $\X$ by $d_{\X}(\f,\f')=\sqrt{\frac{1}{NT}\sum_{i=1}^{NT}(\f(\x_{i},t_i)-\f'(\x_{i},t_i))^2}$. Since the Gaussian process is sub-Gaussian with respect to the Euclidean metric, $\{Z_{\f},\f\in\Fc\}$ is a zero-mean sub-Gaussian process with respect to distance metric $d_{\X}(\cdot,\cdot)$. Let $D=\sup_{\f,\f'\in\Fc}d_\X(\f,\f')$ and follow Theorem~5.22 in \cite{wainwright2019high}, we have that for any $\eps\in[0,D]$,
    \begin{align}
        \E_{\bsgm}\left[\sup_{\f,\f'\in\Fc}(Z_{\f}-Z_{\f'})\right]\leq2\E_{\bsgm}\left[\underset{\underset{d_\X(\f,\f')\leq\eps}{\f,\f'\in\Fc}}{\sup}(Z_{\f}-Z_{\f'})\right]+32\int_{\eps/4}^D\sqrt{\log N(u;\Fc,d_\X)}du,
    \end{align}
    where $N(u;\Fc,d_\X)$ is the $u$-covering number of function set $\Fc$ and metric $d_\X(\cdot,\cdot)$ following Definition~\ref{def:cover number}. 
    
    The first term in the right hand side above is easy to bound, where we have $\E_\bsgm[\sup_{d_\X(\f,\f')\leq\eps}(Z_{\f}-Z_{\f'})]\leq\E_\bsgm[\sup_{\|\vb\|_2\leq\eps}\bsgm^\top\vb]\leq \E_\bsgm[\sup_{\|\vb\|_2\leq\eps}\|\bsgm\|_2\|\vb\|_2]=\sqrt{NT}\eps$. Now and last, it remains to bound the integral term. Here, $N(u;\Fc,d_\X)$ is the $u$-covering number of function set $\Fc$ with respect to distance metric $d_\X$, and $\f\in\Fc$ is a combination function of $\phi\in\Phi, \bho\in\Omega^K, \A\in\Ac$ and $\h\in\Hc^T$. Since $\Ac$ is a discrete set with cardinality $|\Ac|=K^T$. Let $\Fc^{\A}$ be the function set given clustering matrix $\A$. Then we have $\log N(u;\Fc,d_\X)\leq T\log K+\max_{\A\in\Ac}\log N(u;\Fc^{\A},d_\X)$. For any $\f,\f'\in\Fc^\A$, we have
    % We decompose it into covering numbers of function sets $\Hc,\Omega$, and $\Phi$. 
    \begin{align}
        d_\X(\f,\f')&=\sqrt{\frac{1}{NT}\sum_{i=1}^{NT}\left(\f(\x_{i},t_i)-\f'(\x_{i},t_i)\right)^2}\\
        &=\sqrt{\frac{1}{NT}\sum_{t=1}^{T}\sum_{i=1}^N\left(f_t(\x_{t,i})-f'_{t}(\x_{t,i})\right)^2}\\
        &=\sqrt{\frac{1}{NT}\sum_{t=1}^T\sum_{i=1}^N\left(h_t\circ\omega_{A(t)}\circ\phi(\x_{t,i})-h'_t\circ\omega_{A(t)}'\circ\phi'(\x_{t,i})\right)^2}\\
        &\leq\sqrt{\frac{1}{NT}\sum_{t=1}^T\sum_{i=1}^N\left(h_t\circ\omega_{A(t)}\circ\phi(\x_{t,i})-h'_t\circ\omega_{A(t)}\circ\phi(\x_{t,i})\right)^2}\label{eq:h}\\
        &+\sqrt{\frac{1}{NT}\sum_{t=1}^T\sum_{i=1}^N\left(h_t'\circ\omega_{A(t)}\circ\phi(\x_{t,i})-h'_t\circ\omega'_{A(t)}\circ\phi(\x_{t,i})\right)^2}\label{eq:w}\\
        &+\sqrt{\frac{1}{NT}\sum_{t=1}^T\sum_{i=1}^N\left(h_t'\circ\omega'_{A(t)}\circ\phi(\x_{t,i})-h'_t\circ\omega_{A(t)}'\circ\phi'(\x_{t,i})\right)^2}\label{eq:phi}.
    \end{align}
    Let $\X_t=\{\x_{t,i}\}_{i=1}^N$ denote the training inputs of $t_\text{th}$ task with $N$ samples, and $\X_{\Ic_k}=\bigcup_{t\in\Ic_k}\X_t$ denote the training inputs of $k_{th}$ cluster, where $\Ic_k,k\in[K]$ are disjoint sets satisfying $\bigcup_{k\in[K]}\Ic_k=[T]$ and  $\Ic_k=\{t:A_{t,k}=1,t\in[T]\}$. Cluster $k$ contains of $N_k=|\Ic_k|\cdot N$ samples. Then we have
    \begin{align*}
        (\ref{eq:h})&=\sqrt{\frac{1}{T}\sum_{t=1}^T\frac{1}{N}\sum_{i=1}^N\left(h_t\circ\omega_{A(t)}\circ\phi(\x_{t,i})-h'_t\circ\omega_{A(t)}\circ\phi(\x_{t,i})\right)^2}\leq{\frac{1}{T}\sum_{t=1}^Td_{\omega_{A(t)}\circ\phi(\X_t)}}(h_t,h_t')\\
        % (\ref{eq:w})&\leq\Gamma^2{\frac{1}{T}\sum_{t=1}^T\frac{1}{N}\sum_{i=1}^N\left(\omega_{A(t)}\circ\phi(\x_{t,i})-\omega_{A(t)}'\circ\phi(\x_{t,i})\right)^2}=\Gamma^2{\frac{1}{T}\sum_{t=1}^Td^2_{\phi(X_t)}}(\omega_{A(t)},\omega'_{A(t)})\\
        (\ref{eq:w})&\leq\Gamma\sqrt{\frac{1}{K}\sum_{k=1}^K\frac{1}{N_k}\sum_{i=1}^{N_k}\left(\omega_{k}\circ\phi(\x_{k,i})-\omega_{k}'\circ\phi(\x_{k,i})\right)^2}\leq{\frac{\Gamma}{K}\sum_{k=1}^Kd_{\phi(\X_{\Ic_k})}}(\omega_{k},\omega'_{k})\\
        (\ref{eq:phi})&\leq\Gamma^2\sqrt{\frac{1}{NT}\sum_{t=1}^T\sum_{i=1}^N\left(\phi(\x_{t,i})-\phi'(\x_{t,i})\right)^2}=\Gamma^2d_\X(\phi,\phi').
    \end{align*}
    Given inputs $\X$, and clustering matrix $\A$, we consider the $\eps'$-covers over function spaces $\Hc,\Omega,\Phi$ corresponding to its specific metric $d(\cdot,\cdot)$. 
    \begin{align}
        d_\X(\f,\f')&\leq\frac{1}{T}\sum_{t=1}^Td_{\omega_{A(t)}\circ\phi(\X_t)}(h_t,h_t')+\frac{\Gamma}{K}\sum_{k=1}^Kd_{\phi(\X_{\Ic_k})}(\omega_k,\omega_k')+\Gamma^2d_\X(\phi,\phi')\\
        &\leq(1+\Gamma+\Gamma^2)\eps'.
    \end{align}
    Firstly, consider about the $\eps'$-cover of function set $\Phi$ with respect to $d_\X$, and the covering number is $N(\eps';\Phi,d_\X)$. For any chosen function $\phi$ in this cover, letting $\phi(\X)$ be new inputs, we cluster these inputs to $\phi(\X_{\Ic_k}), k\in[K]$ with respect to given $\A$. Then in cluster $k$, the $\eps'$-covering number of function set $\Omega$ is $N(\eps';\Omega,d_{\phi(\X_{\Ic_k})})$. Since we assume $K$ clusters in total, and each cluster satisfies the covering constraint, therefore, the $\eps'$-covering number for $\bho\in\Omega^K$ with respect to $d_{\phi(\X)}(\cdot,\cdot)$ is $\Pi_{k\in[K]}N(\eps';\Omega,d_{\phi(\X_{\Ic_k})})$. Similarly, for any chosen $\bho,\phi$, the $\eps'$-covering number of $\h\in\Hc^T$ with respect to metric $d_{\bho\circ\phi(\X)}(\cdot,\cdot)$ is $\Pi_{t\in[T]}N(\eps';\Hc,d_{\omega_{A(t)}\circ\phi(\X_t)})$. Now, combine them together and consider all the possibilities in $\eps'$-covers of $\phi,\bho$ and $\h$. Recalling that $\log N(u;\Fc,d_\X)\leq T\log K+\max_{\A\in\Ac}\log N(u;\Fc^{\A},d_\X)$ and letting $\eps'=\frac{u}{1+\Gamma+\Gamma^2}$, we have
    \begin{align*}
        \log N(u;\Fc,d_\X)&\leq T\log K+\max_{\A\in\Ac}\log N((1+\Gamma+\Gamma^2)\eps';\Fc^{\A},d_\X)\\
        &\leq T\log K+\log N(\eps';\Phi,d_\X)\\
        &+\sup_{\phi\in\Phi,\bho\in\Omega^K,\A\in\Ac}\left(\sum_{t\in[T]}\log N(\eps';\Hc,d_{\omega_{A(t)}\circ\phi(\X_t)})+ \sum_{k\in[K]}\log N(\eps';\Omega,d_{\phi(\X_{\Ic_k})})\right)\\
        &\leq T\log K+\log N(\eps';\Phi,d_\X)\\
        &+\sup_{\phi\in\Phi,\bho\in\Omega^K,\A\in\Ac}\left(\sum_{t\in[T]}\log N(\eps';\Hc,d_{\omega_{A(t)}\circ\phi(\X_t)})\right)+\sup_{\phi\in\Phi,\A\in\Ac}\left( \sum_{k\in[K]}\log N(\eps';\Omega,d_{\phi(\X_{\Ic_k})})\right)\\
        &\leq T\log K+\log N(\eps';\Phi,d_\X)\\
        &+T\cdot\sup_{\phi\in\Phi,\omega\in\Omega,t\in[T]}\log N(\eps';\Hc,d_{\omega\circ\phi(\X_t)})+\sup_{\phi\in\Phi,\A\in\Ac}\left( \sum_{k\in[K]}\log N(\eps';\Omega,d_{\phi(\X_{\Ic_k})})\right)\\
    \end{align*}
    
    Inspired by \cite{tripuraneni2020theory} and from the Sudakov minoration theorem (Theorem~5.30) and Lemma~5.5 in \cite{wainwright2019high}, for any $\eps'>0$, we have that
    \begin{align}
        \sqrt{\log N(\eps';\Phi,d_\X)}&\leq\frac{2}{\eps'}\E\left[\sup_{\phi\in\Phi}\frac{1}{\sqrt{NT}}\sum_{i=1}^{NT}\sigma_i\cdot \phi(\x_{i}')\right]=\frac{2\sqrt{NT}}{\eps'}\hat\Rc_{\X}(\Phi)\\
        \sqrt{\log N(\eps';\Hc,d_{\X'_t})}&\leq\frac{2}{\eps'}\E\left[\sup_{h\in\Hc}\frac{1}{\sqrt{N}}\sum_{i=1}^N\sigma_i\cdot h(\x_{t,i}')\right]=\frac{2\sqrt{N}}{\eps'}\hat\Rc_{\X_t'}(\Hc)\\
        \sqrt{\log N(\eps';\Omega,d_{\X''_k})}&\leq\frac{2}{\eps'}\E\left[\sup_{\omega\in\Omega}\frac{1}{\sqrt{N_k}}\sum_{i=1}^{N_k}\sigma_i\cdot \omega(\x_{k,i}')\right]=\frac{2\sqrt{N_k}}{\eps'}\hat\Rc_{\X_k''}(\Omega)
    \end{align}
    where $\X_t':=\omega\circ\phi(\X_t)$ and $\X_k'':=\phi(\X_{\Ic_k})$. Hence, the integral term is bounded by
    \begin{align}
        \int_{\eps/4}^D\sqrt{\log N(u;\Fc,d_\X)}du&\leq\sqrt{T\log K}\cdot(D-\eps/4)\\
        &+2\sqrt{NT}(1+\Gamma+\Gamma^2)\int_{\eps/4}^D\frac{1}{u}du\cdot\left(\hat\Rc_\X(\Phi)+\bar\Rc_{\X'_t}(\Hc)+\bar\Rc_{\X''}(\Omega)\right)
    \end{align}
    Combining all together, we have with probability at least $1-\delta$
    \begin{align}
        \Lc(\hat\f)-\Lc(\f^\star)&\leq8L\hat\Rc_{\X}(\Fc)+3\sqrt{\frac{2\log\frac{4}{\delta}}{NT}}\\
        &\leq16L\left(\eps+\frac{D}{2}\sqrt{\frac{\log K}{N}}+32(1+\Gamma+\Gamma^2)\log\frac{4D}{\eps}\cdot\left(\hat\Rc_\X(\Phi)+\bar\Rc_{\X'_t}(\Hc)+\bar\Rc_{\X''}(\Omega)\right)\right)+3\sqrt{\frac{2\log\frac{4}{\delta}}{NT}}\\
        &\leq
    \end{align}
    
    
    
    \end{proof}

==> app/proof_fairness.tex <==
\section{Fairness Drawbacks of Underparameterized Representations}\label{sec unfair}

Let us start by describing the data distribution we consider. We consider a linear model with $T=T_0+T_1$ tasks parameterized by vectors $\bt^\st_{t}\in\R^p$. We assume that each vector lies on one of the two orthogonal subspaces. We denote these subspaces via the row space of the matrices $\B_0\in\R^{r\times d}$ and $\B_1\in\R^{r_1\times d}$ where $\B_0\B_0^\top=\B_1\B_1^\top=\Iden$ and $\B_0\B_1^\top=0$. Without losing generality, let first $T_0$ tasks lie on $\B_0$ and last $T_1$ lie on $\B_1$. Let $\alpha_t$ be the clustering/pathway choice $\alpha_t=0$ for $t\leq T_0$ and $\alpha_t=1$ for $t>T_0$. Thus, for some $(\h^\st_t)_{t=1}^T$, we have $\bt^\st_{t}=\B_{\alpha_t}^\top \h^\st_{t}$ for all $t\in[T]$.


\textbf{Datasets:} We assume that $T_0\geq T_1$, thus, $\B_0$ and $\B_1$ corresponds to majority and minority task clusters respectively. $\Sc_t$ denote the training dataset of task $t$. We assume linear labeling functions where i.i.d.~samples are given by $y_{ti}=\li\bt^\st_{t},\x_{ti}\ri+z_{ti}$ for $i\in [N]$. Here input features $\x_{ti}$ and noise $z_{ti}$ are zero-mean and independent with $\order{1}$ subgaussian norm. Let $\x^{kt}_i$ has identity covariance and fix the noise variance to $\E[z_{ti}^2]=\sigma^2$. Let $\Sc=\bigcup_{t=1}^T \Sc_t$.

Fix $C\geq 1$. We solve the empirical risk minimization over parameters $\fb=\{\B,(\h_t)_{t=1}^T\}$ over hypothesis class $\Fc=\{\B,\h_t\big| \B\B^\top=\Iden,~\tn{\h_t}\leq C\}$ where $\B\in\R^{r\times d}$ is the shared representation as follows%Define the empirical and population risks
\begin{align}
\hat \fb=\arg\min_{\fb}\Lch(\fb_{ti})=\frac{1}{TN} \sum_{t=1}^T\sum_{i=1}^N(y_{ti}-\h_t^\top \B\x_{ti})^2.\label{vanilla MTL}
%\Lch(f)=\Lch_1(f)+\Lch_2(f),\quad 
\end{align}
%$\Lc(\fb)=\E[\Lch(\fb)]$ and 
Let $\Rc(\fb)=\Lc(\fb)-\sigma^2$ be the task-averaged excess population risk. Define the population excess risks of respective subspaces as follows
\begin{align}
\Rc_0(\fb)=\frac{1}{T_0} \sum_{t=1}^{T_0}\E[(y_{ti}-\h_t^\top \B\x_{ti})^2]-\sigma^2,\quad\Rc_1(\fb)=\frac{1}{T_1} \sum_{t=T_0+1}^T\E[(y_{ti}-\h_t^\top \B\x_{ti})^2]-\sigma^2,
\end{align}
 satisfying $\Rc(\fb)=\Rc_0(\fb)+\Rc_1(\fb)$. Let $(x)_+:=\max(x,0)$. Given any $q\geq 0$, define spectrum tail of a PSD matrix $\A\in\R^{d\times d}$ to be 
 \[
 \text{tail}(\X,q)=\sum_{i=\lceil (d-q+1)_+\rceil}^d \la_i(\A)
 \]
 where $\la_i$ is the $i$'th largest eigenvalue. We have the following control on the generalization risk of minority/majority tasks. 
 
 \begin{theorem}\label{thm unfair}Consider the vanilla multitask learning approach \eqref{vanilla MTL}. Assume both clusters are diverse in the sense that, for some $\xi>0$, task covariances% (with proper $r\times r,r_1\times r_1$dimensions)
 \[
 \Hb_0=\frac{1}{T_0}\sum_{t=1}^{T_0} \h_t\h_t^\top,~ \Hb_1=\frac{1}{T_1}\sum_{t=T_0+1}^{T} \h_t\h_t^\top.%\quad \text{ and }\quad\xi\Iden/r_1\leq\preceq \Xi\Iden/r_1.
 \]
Assume $ \Xi\Iden /r\succeq\Hb_0\succeq \xi\Iden /r$. Let $\fbb=\{\Bb,(\hb_t)_{t=1}^T\}$ be the population minima obtained as $N\rightarrow \infty$. The majority/minority excess risks obey
 \[
\text{Majority:}~\Rc_0(\fb)\leq \frac{\Xi T_1}{\xi T},\quad \text{Minority:}~\Rc_1(\fb)\geq \text{tail}(\Hb_1,r_1-rT_1/\xi T_0).
 \] 
 \end{theorem}
 %. Suppose $\|\Hb_1\|\leq \Xi_1$ for some $\Xi_1>0$.
 \begin{corollary} Consider the setting of Theorem \ref{thm unfair}. We have that
 \[
\lim_{T_1/T_0\rightarrow0} \Rc_0(\fb)=0,\quad \lim_{rT_1/T_0\rightarrow0} \Rc_1(\fb)=1.
 \]
Additionally suppose $\|\Hb_1\|\leq \Xi_1$ for some constant $\Xi_1>0$. Then $\underset{rT_1/r_1T_0\rightarrow0}{\lim} \Rc_1(\fb)=1$.
 \end{corollary}
 \textbf{Interpretation:} The majority excess risk is tightly upper bounded by the relative fraction of the minority tasks $T_1/T_0$. On the other hand, minority risk is lower bounded by the eigen-tail of the task covariance in terms of $T_1/T_0$. Specifically, as $T_1/T_0$ decreases, we prove that optimal representation is less and less aligned with minority subspace. In the proper limit, minority tasks achieve the trivial risk $\Rc_1(\fb)=1$ that corresponds to making zero prediction $\hat y= 0$. Finally, the limit $rT_1/r_1T_0\rightarrow0$ is a much milder condition compared to $rT_1/T_0\rightarrow0$. This milder condition can be interpreted as follows: Majority tasks have $T_0/r$ label energy per subspace dimension. In contrast, minority tasks have $T_1/r_1$ label energy per dimension. When majority energy-per-dimension dominates minority, all subspace dimensions of the representations are assigned to majority to minimize task-averaged risk.
 % decreases. In fact, in the limit $T .  %As soon as minorities are negligible fraction, the risk over majority tasks is small.
 
 \subsection{Proof of Theorem \ref{thm unfair}}
 \begin{proof} Let $\Pb_k=\B_k{\Bb}^\top{\Bb}\B_k^\top$ be the projection of $\Bb$ onto $\B^k$. Observe that 
 \begin{align}
& \tr{\Pb_0}+\tr{\Pb_1}=\tr{{\Bb}^\top{\Bb}(\B_0^\top\B_0+\B_1^\top\B_1)}\leq \tr{{\Bb}^\top{\Bb}}\leq r\implies\\
&\tr{\Iden-\Pb_0}+\tr{\Iden-\Pb_1}\geq r_1.\label{excess trace}
 \end{align}
Given $\Bb$, the excess population risk (after subtracting the noise variance) takes the form% takes the formSince $\Bb$ is the population minima, we have that
\begin{align}
\Lc(\fbb)-\sigma^2&=  \frac{1}{T}\sum_{t=1}^{T}\min_{\h_t}\tn{ {\Bb}^\top\h_t-\bt^\st_t}^2=\frac{1}{T}\sum_{t=1}^{T}\tn{(\Iden-{\Bb}^\top{\Bb})\bt^\st_t}^2\\
&=\frac{T_0}{T}\tr{\B_0^\top\Hb_0\B_0(\Iden-{\Bb}^\top{\Bb})}+\frac{T_1}{T}\tr{\B_1^\top\Hb_1\B_1(\Iden-{\Bb}^\top{\Bb})}\\
&=1-[\frac{T_0}{T}\tr{\Hb_0\B_0{\Bb}^\top{\Bb}\B_0^\top}+\frac{T_1}{T}\tr{\Hb_1\B_1{\Bb}^\top{\Bb}\B_1^\top}]\\
&=\frac{T_0}{T}\tr{\Hb_0(\Iden-\Pb_0)}+\frac{T_1}{T}\tr{\Hb_1(\Iden-\Pb_1)}.
\end{align}%state a slightly more general result 
Set $\rho=\tr{\Iden-\Pb_0}/r$. To better capture the dependencies in terms of minority covariance, also assume $\Hb_1=\frac{r_1}{T_1}\sum_{t=T_0+1}^{T} \h_t\h_t^\top\succeq\xi_1\Iden$. We will end up setting $\xi_1=0$ eventually. Recalling above \eqref{excess trace} and applying Von Neumann's trace inequality, we find
\begin{align}
\Lc(\fbb)-\sigma^2&\geq \frac{\xi}{Tr} T_0\tr{\Iden-\Pb_0}+\frac{\xi_1}{Tr_1} T_1\tr{\Iden-\Pb_1}\\
&\geq \frac{\xi T_0\rho}{T} +\frac{\xi_1T_1 (1-\rho r/r_1)_+}{T}.
%1-\frac{T_0\Xi\tr{\Pb_0}}{Tr}-\frac{T_1\Xi\tr{\Pb_1}}{Tr_1}\\&\geq 1-\frac{T_0\Xi\tr{\Pb_0}}{Tr}-\frac{T_1\Xi(r-\tr{\Pb_0})}{Tr_1}
\end{align}
Now, consider the suboptimal solution $\tilde{\fb}$ which picks $\B=\B_0$, $\h_t=\h_t^\st$ for $t\leq T_0$ and $\h_t=0$ for $t>T_0$. This solution exactly achieves 
\[
\Lc(\tilde{\fb})-\sigma^2\leq \frac{T_1}{T}.
\]
Putting things together, we found
\[
\xi T_0\rho+\xi_1T_1 (1-\rho r/r_1)_+\leq T_1.
\]
This in turn implies
\[
\rho \leq  \frac{T_1(1-\xi_1(1-\rho r/r_1)_+)}{\xi T_0}\leq \frac{T_1}{\xi T_0}.
\]
Through this, we shall lower bound minority risk and upper bound majority risk. Using \eqref{excess trace} and observing $\tr{\Iden-\Pb_1}\geq (r_1-r\rho)_+\geq (r_1-rT_1/\xi T_0)_+$, minority excess risk is given by
\[
\Rc_1(\fbb)=\tr{\Hb_1(\Iden-\Pb_1)}\geq \text{tail}(\Hb_1,r_1-rT_1/\xi T_0)
\]
where we again applied Von Neumann's trace inequality. On the other hand, majority excess risk obeys
\[
\Rc_0(\fbb)=\frac{T_0}{T}\tr{\Hb_0(\Iden-\Pb_0)}\leq \Xi \rho T_0/T\leq \frac{\Xi T_1}{\xi T}.
\]
\end{proof}



%Set $\rho=\tr{\Iden-\Pb_0}/r$. To state a more general result in terms of minority covariance, also assume $\Hb_1=\frac{r_1}{T_1}\sum_{t=T_0+1}^{T} \h_t\h_t^\top\succeq\xi_1\Iden$. We will end up setting $\xi_1=0$ eventually. Recalling above \eqref{excess trace} and applying Von Neumann's trace inequality, we find
%\begin{align}
%\Lc(\fbb)-\sigma^2&\geq \frac{\xi}{Tr} T_0\tr{\Iden-\Pb_0}+\frac{\xi_1}{Tr_1} T_1\tr{\Iden-\Pb_1}\\
%&\geq \frac{\xi T_0\rho}{T} +\frac{\xi_1T_1 (1-\min(\rho r/r_1,1))}{T}.
%%1-\frac{T_0\Xi\tr{\Pb_0}}{Tr}-\frac{T_1\Xi\tr{\Pb_1}}{Tr_1}\\&\geq 1-\frac{T_0\Xi\tr{\Pb_0}}{Tr}-\frac{T_1\Xi(r-\tr{\Pb_0})}{Tr_1}
%\end{align}
%Now, consider the suboptimal solution $\tilde{\fb}$ which picks $\B=\B_0$, $\h_t=\h_t^\st$ for $t\leq T_0$ and $\h_t=0$ for $t>T_0$. This solution exactly achieves 
%\[
%\Lc(\tilde{\fb})-\sigma^2\leq \frac{T_1}{T}.
%\]
%Putting things together, we found
%\[
%\xi T_0\rho+\xi_1T_1 (1-\min(\rho r/r_1,1))\leq T_1.
%\]
%This in turn implies
%\[
%\rho \leq  \frac{T_1(1-\xi_1)}{\xi T_0-\xi_1T_1 r/r_1}\leq \frac{T_1}{\xi T_0}.
%\]
%Through this, we shall lower bound minority risk and upper bound majority risk. Using \eqref{excess trace} and observing $\tr{\Iden-\Pb_1}\geq r_1-\min(r\rho,r_1)\geq r_1-\min(rT_1/\xi T_0,r_1)$, minority excess risk is given by
%\[
%\Rc_1(\fbb)-\sigma^2=\tr{\Hb_1(\Iden-\Pb_1)}\geq \tr{\Hb_1(r_1-r\rho)}
%\]
%where we again applied Von Neumann's trace inequality.

==> app/proof_hierarchy.tex <==
\section{Proofs/Corollaries in Section~\ref{hierarchy}}\label{app:proof hierarchy}


==> sec/background.tex <==
\onecolumn
\section*{Background}

\subsection{Multitask learning}
\textbf{Notation.} Let $\|\cdot\|$ denote the $\ell_2$-norm of a vector, and $[L]$ denote the set $\{1,2,\dots,L\}$.

Consider a multitask learning (MTL) setup. Let $\Xc$ denote the domain of raw input features.
Suppose we have $T$ tasks with data distribution $\{\Dc_t\}_{t=1}^T$. During training, we are given $T$ training datasets $\{\Sc_t\}_{t=1}^T$. Here, $\Sc_t$ are i.i.d drawn from its corresponding distribution $\Dc_t$. Let $\Sc_t=\{(\x_{t,i},y_{t,i})\}_{i=1}^{N_t}$, where $(\x,y)\in(\Xc,\R)$ is a input-label pair, and $N_t$ and $\bar{N_t}$ are training and validation sample numbers of $t_{\text{th}}$ task. 


Let $\Zc$ be latent feature space. We define the hypothesis sets of \emph{feature extractors} $\Phi:\Xc\rightarrow\Zc$ and \emph{model headers} $\Hc:\Zc\rightarrow\R$. That it, the function $\phi\in\Phi$ maps raw features in $\Xc$ to a latent space $\Zc$ and the function $h\in\Hc$ maps latent features in $\Zc$ to a prediction in $\R$. We construct a hypothesis $f:\Xc\rightarrow\R$ by picking $\phi\in\Phi$ and $h\in\Hc$ and setting $f=h\circ\phi$. In the multitask learning setting, $T$ tasks share the same feature extraction function $\phi$ but each learns to find its specific header $h_t,t\in[T]$. Then, given the loss function $\ell(\hat{y},y)$, the multitask learning problem can be formulated as follows. 
\begin{align}
    \hat\phi,\{\hat h_t\}_{t=1}^T=\underset{\phi\in\Phi,h_t\in\Hc}{\arg\min}\frac{1}{T}\sum_{t=1}^T\hat\Lc_{\Sc_t}(h_t\circ\phi),~~~\text{where}~~~\hat\Lc_{\Sc_t}(h_t\circ\phi)=\frac{1}{N_t}\sum_{i=1}^{N_t}\ell(h_t\circ\phi(\x_{t,i}),y_{t,i}).
\end{align}
Firstly, compared to individual learning $\Oc(\sqrt{\frac{\log|\Phi|+\log|\Hc|}{N}})$, MTL is sample efficient with sample complexity $\Oc(\sqrt{\frac{\log|\Phi|+T\log|\Hc|}{TN}})$, that is, a task can learn a large model with less samples. Secondly, if the training tasks are highly related, then the knowledge learned from a task benefits the other tasks in better generalization performance. 
However, tasks might also `hurt' each other. Then, instead of using only one $\phi$, we split $T$ tasks into $K$ clusters and learn $K$ different feature extractors $\phi_k,k\in[K]$. 
\begin{align}
    \{\hat\phi_k\}_{k=1}^K,\{\hat h_t\}_{t=1}^T=\underset{\phi_k\in\Phi,h_t\in\Hc}{\arg\min}\frac{1}{T}\sum_{t=1}^T\hat\Lc_{\Sc_t}(h_t\circ\phi_{k_t}),~~~\text{where}~~~\hat\Lc_{\Sc_t}(h_t\circ\phi_{k_t})=\frac{1}{N_t}\sum_{i=1}^{N_t}\ell(h_t\circ\phi_{k_t}(\x_{t,i}),y_{t,i}).
\end{align}
where $k_t\in[K]$ is the cluster ID of tasks $t$. In this case, the sample complexity is around $\Oc(\sqrt{\frac{K\log|\Phi|+T\log|\Hc|}{TN}})$

\begin{align}
    \hat\phi_0,\{\hat\phi_k\}_{k=1}^K,\{\hat h_t\}_{t=1}^T&=\underset{\phi_k\in\Phi,h_t\in\Hc}{\arg\min}\frac{1}{T}\sum_{t=1}^T\hat\Lc_{\Sc_t}(h_t\circ\phi_{k_t}\circ\phi_0),\\
    \text{where}~~~\hat\Lc_{\Sc_t}(h_t\circ\phi_{k_t}\circ\phi_0)&=\frac{1}{N_t}\sum_{i=1}^{N_t}\ell(h_t\circ\phi_{k_t}\circ\phi_0(\x_{t,i}),y_{t,i}).
\end{align}
% \subsection{Personalized representation learning}
% Since in standard MTL problem, all the tasks share the same feature extractor $\phi$. It shows that knowledge learned from a task benefits the other tasks in better performance.
% \subsection{Continual learning}

% \subsection{Transfer learning}
\twocolumn
\newpage

==> sec/cluster.tex <==
\section{Clustering MTL}
We start with a simpler clustering MTL as shown in Fig.~\ref{fig:intro_tree}. Assume we have $T$ tasks, each with distribution $\Dc_t$, training datasets $\Sc_t$ and the same training sample size $N$. In this setting, we assume that we have $K$ clusters (subspaces), and in addition to training a global-shared feature extractor $\phi\in\Phi$, we train $K$ cluster-specific extractors $\omega_k\in\Omega,k\in[K]$. Our goal is to train prediction function for each task with $f_t:=h_t\circ\omega_{A_{tk}}\circ\phi$, where the cluster is parameterized by a clustering matrix $\A\in\Ac\subset\R^{T\times K}$. Let $A_t$ denotes the $t_{\text{th}}$ row and $A
_{t,k}$ denotes the $i_{\text{th}}$ row and $k_{\text{th}}$ column of matrix $\A$. Let $\bho:=(\omega_1,\dots,\omega_K)\in\Omega^K$, and $\h:=(h_1,\dots,h_T)\in\Hc^T$. Hence the simplest clustering MTL problem of $K$-degree can be formulated as

\begin{align}
    \hat\phi,~\hat\A,~\hat\bho,~\hat\h=\underset{\underset{\bho\in\Omega^K,\h\in\Hc^T}{\phi\in\Phi,\A\in\Ac}}{\arg\min}\frac{1}{NT}\sum_{t=1}^{T}\sum_{i=1}^{N}\ell(h_t\circ\omega_{A(t)}\circ\phi(\x_{t,i}),y_{t,i})\label{formula:cluster}
\end{align}

\noindent$\bullet$~\textbf{Hard clustering} is to assign each task to one of the $K$ clusters, that is, $\A_t(t\in[T])$ are one-hot vectors, and the index of nonzero entry determines the cluster membership. Therefore, $\A$ has finite search space with $|\Ac|=K^T$. In (\ref{formula:cluster}), $A(t)$ returns the index of the nonzero element of $\A_t$, which is the cluster ID of $t_{\text{th}}$ task.
% It can also be seen as the number of achievable paths.

% \noindent$\bullet$~\textbf{Soft clustering} assumes 


\begin{assumption}\label{assum:lipschitz} $\Phi$, $\Omega$ and $\Hc$ are all sets of $\Gamma$-Lipschitz functions.
\end{assumption}
\begin{theorem} Let $\hat \f$ be the solution of (\ref{formula:cluster}) and $\f^\star$ be the population risk minimizer of (\ref{formula:cluster}), that is with $N=\infty$. Suppose Assumption~\ref{assum:lipschitz} holds. Let $\ell(\hat y,y)$ be an $L$-Lipschitz function taking values in $[0,1]$. Denote $\Lc(\f):=\frac{1}{T}\sum_{t=1}^T\Lc_{\Dc_t}(f_t)$ and $\hat\Lc(\f):=\frac{1}{NT}\sum_{t=1}^T\sum_{i=1}^N\ell(f_t(\x_{t,i}),y_{y,i})$.
\begin{align} 
    \Lc(\hat\f)-\Lc(\f^\star)\leq
\end{align}
\end{theorem}




==> sec/exp.tex <==
\section{Experiments}

==> sec/organization.tex <==

\onecolumn
\section*{Organization}
%\begin{enumerate}
%    \item Main result: Multipath MTL 
%    \item Extensions: transfer learning; different depths; continuous paths; 
%    \item Experiments: CtRL
%    \item Further work: sparse MTL
%\end{enumerate}
\subsection{Main result - Multipath MTL}
Consider a MTL problem with $T$ tasks and each task has $N$ training samples. Assume we have a supernet as depicted in Figure~\ref{fig:intro} with $L$ layers, and each task is trained to find a subnetwork with depth $L$. 
\[
\Lc-\Lc^\star\leq C_1\sqrt{\frac{\log|\Ac|}{N}}+C_2\log NT\cdot\left(\bar\Rc(\Hc)+\red{\sum_{i\in[L]}\bar\Rc(\Psi_i)}\right)+\delta
\]
\subsection{Extensions - Transfer learning}
Let $\bar\phi$ and $\phi^\#$ be empirical and population solutions of multipath MTL, which are trained with source data, and let $\hat\alpha$, $\alpha^\star$, $\hat h$, $h^\star$ be the empirical and population solutions of path selection and head with respect to $\bar\phi$ and $\phi^\#$.
\begin{align*}
    L(\bar\phi,\hat h, \hat\alpha)-L(\phi^\#,h^\star,\alpha^\star)\leq \underset{\leq 4\Rc_N(\Hc)+\sqrt{\log|\Ac|/N}}{\underbrace{L(\bar\phi,\hat h,\hat\alpha)-L(\bar\phi,h',\alpha')}}+\underset{\text{model distance}}{\underbrace{L(\bar\phi,h',\alpha')-L(\phi^\#,h^\star,\alpha^\star)}}\left(+\underset{\text{distribution distance}}{\underbrace{L(\phi^\#,h^\star,\alpha^\star)-L(\phi^\star,h^\star)}}\right)
\end{align*}

\begin{definition} [Model distance - representation mismatch]
    Assume we have two multipath basemodels. 
    \begin{align*}
        d(\phi,\phi'):=\max_{\alpha'\in\Ac}\min_{\alpha\in\Ac}\E_{\x}\|\phi_{\alpha}(\x)-\phi'_{\alpha'}(\x)\|
    \end{align*}
    OR
    \begin{align*}
    	d(\phi,\phi')=\sup_{\alpha'\in\Ac,h'\in\Hc}\inf_{\alpha\in\Ac,h\in\Hc}\E\left[\ell(\h\circ\phi_{\alpha}(\x)-\ell(\h'\circ\phi'_{\alpha'}(\x)))\right]
    \end{align*}

\end{definition}
\subsection{Experiments}
\begin{enumerate}
    \item Subspace experiments with two hidden linear layers. Let $\B^{(1)}\in\R^{d\times R}$, $\B^{(2)}\in\R^{R\times r}$ be two hidden layers and $\bho\in\R^{r}$ be the fully-connected head. Then 
    \[
        y=\bho_t\B^{(2)}_k\B^{(1)}\x
    \]
\end{enumerate}

\twocolumn
\newpage

==> sec/related.tex <==
\section{Related Works}
%Our work establishes generalization guarantees for multipath multitask learning and also shows theoretical benefits in transfer learning when adapting to new tasks. 
Our work is related to a large body of literature spanning efficient architectures for MTL and continual learning as well as statistical learning guarantees for MTL. Due to space limitations, we restrict our attention to the closely related works, and defer the more detailed discussion of prior art to the supplementary material.% provides a more extensive discussion.% of   These connections are discussed below.

%/Meta-Learning/Representation Learning/Transfer Learning
\noindent $\bullet$ \textbf{Multitask Representation Learning.} While MTL problems admit multiple approaches, an important idea is building shared representations to embed tasks in a low-dimensional space \cite{zhang2021survey,thrun2012learning,baxter2000model}. After identifying this low-dimensional representation, new tasks can be learned in a sample efficient fashion inline with the benefits of deep representations in modern ML applications. While most earlier works focus on linear models, \cite{maurer2016benefit} provides guarantees for general hypothesis classes through empirical process theory improving over \cite{baxter2000model}. More recently, there is a growing line of work on multitask representations that spans tighter sample complexity analysis \cite{du2020few,kong2020meta,xu2021representation,lu2021power}, convergence guarantees \cite{collins2022maml,ji2020convergence,collins2021exploiting}, lifelong learning \cite{xu2022statistical,li2022provable}, and decision making problems \cite{yang2020impact,cheng2022provable}. Closest to our work is \cite{tripuraneni2021provable} which provides tighter sample complexity guarantees compared to \cite{maurer2016benefit}. Our problem formulation generalizes prior work (that are mostly limited to single shared representation) by allowing deep compositional representations computed along supernet pathways. To overcome the associated technical challenges, we develop multilayer chain rules for Gaussian Complexity, introduce new notions to assess the quality of supernet representations, and develop new theory for linear representations.

%To the best of our knowledge, prior theory is restricted to a single shared representation 
%Importantly, all prior works focus on a single shared representation 

%The the statistical benefits of these shared representations.

%Accomplishing this would enableOnce this is accomplished, each task can be learned sample efficiently.%Theoretical aspects of MTL and transfer learning have been investigated throughly over the years
%\cite{tripuraneni2021provable} provides theoretical learning guarantee for linear representation. 


%\noindent$\bullet$ \textbf{Personalized Federated Learning.}

\noindent $\bullet$ \textbf{Related ML Architectures and Systems.} While traditional machine learning models tend to be good at a handful of tasks, next-generation of neural architectures are expected to excel at a diverse range of tasks while allowing for multiple input modalities. To this aim, task-specific representations can help address both computational and data efficiency challenges. Recent works \cite{fifty2021efficiently,yao2019hierarchically,vuorio2019multimodal,mansour2020three,tan2022towards,ghosh2020efficient,collins2021exploiting} propose hierarchical/clustering approaches to group tasks in terms of their similarities. In the context of lifelong learning, PathNet and PackNet \cite{fernando2017pathnet,mallya2018packnet} propose to embed many tasks into the same network to facilitate sample/compute efficiency. PathNet as well as SNR \cite{ma2019snr} propose methods to identify pathways/routes for individual tasks and efficiently compute them over the conditional subnetwork. With the advent of large language models, conditional computation paradigm is witnessing a growing interest with architectural innovations such as muNet, GShard, Pathways, and PaLM \cite{gesmundo2022evolutionary,gesmundo2022munet,barham2022pathways,pathways,lepikhin2020gshard,chowdhery2022palm} and provide a strong motivation for theoretically-grounded \MP MTL methods.

% that solve a diverse range of tasks while also allowing for multimodal 

% of work to ensure next-generation neural network architectures are capable of accomplishing multiple tasks and consuming multimodal information.
%enable efficient deployment of large neural nets Our work is influenced by recent architectural 



==> sec/setup.tex <==
\subsection{Multipath multitask learning}
In this section, we discuss about the multipath multitask learning as shown in Fig.~\ref{fig:intro_grid}. Suppose we have $T$ tasks with data distribution $\{\Dc_t\}_{t=1}^T$. During training, we are given $T$ training datasets $\{\Sc_t\}_{t=1}^T$. Here, $\Sc_t$ are i.i.d drawn from its corresponding distribution $\Dc_t$. Let $\Sc_t=\{(\x_{t,i},y_{t,i})\}_{i=1}^{N}$, where $(\x,y)\in(\Xc,\R)$ is an input-label pair, and $N$ is the number of training samples of $t_{\text{th}}$ task. 

% We define the hypothesis set of feature extractors $\Phi:\Xc\rightarrow\Zc$ and task-specific heads $\Hc:\Zc\rightarrow\R$. That it, the function $\phi\in\Phi$ maps the raw feature in $\Xc$ to a latent feature in $\Zc$ and $h\in\Hc$ maps the latent feature in $\Zc$ to a prediction in $\R$. 


% Here, we consider the multitask problem that different tasks can learn to find its specific submodels. 

% Assume we are given a loss function $\ell(\hat y,y)$ and define the training risk over dataset $\Sc$ as $\hat\Lc_{\Sc}(f):=\frac{1}{|\Sc|}\sum_{i=1}^{|\Sc|}\ell(f(\x_i),y_i)$ where $|\Sc|$ is the cardinality of the set, and the test risk over distribution $\Dc$ as $\Lc_{\Dc}(f):=\E_{\Dc}[\ell(f(\x_i),y_i)]$, where we have $\Lc_{\Dc}(f)=\E_{\Dc}[\hat\Lc_{\Sc}(f)]$.

Suppose we have a supernet with $L$ layers (excluding the last layer) and each has $D_l$ modules, $l\in[L]$. We assume that modules in the same layer have the same hypothesis set and let $\Psi_i$ be the hypothesis set of modules in $i_{\text{th}}$ layer, $i\in[L]$. As shown in Fig.~\ref{fig:intro}, a supernet can be seen as a directed-graph. Denote $\Ac$ as a set of all achievable paths, and $\alpha\in\Ac$ be a specific path. Taking Fig.~\ref{fig:intro_grid} as an example, we can mark the paths as $\alpha_{\text{red}}=((1,2),(2,3))$, $\alpha_{\text{green}}=((1,2),(2,4),(3,3))$ and $\alpha_{\text{black}}=((1,1),(2,2),(3,3),(4,3),(5,1))$. $|\Ac|$ is the number of achievable paths. To simplify, we assume that all the tasks aim to find a path with length $L$, therefore, in Fig.~\ref{fig:intro_grid}, $|\Ac|=\prod_{l\in[L]}D_l$, while in Fig.~\ref{fig:intro_tree} with degree $K$, $|\Ac|=K^{L-1}$. Define the path-dependent feature extractor as $\phi_\alpha$, where $\phi_\alpha$ is a combination of functions $\{\psi_{i,j}:(i,j)\in\alpha\}$. Then in Fig.~\ref{fig:intro_grid}, we have $\phi_{\alpha_\text{green}}:=\psi_{3,3}\circ\psi_{2,4}\circ\psi_{1,2}$. 
Our goal is to train a prediction function for each task with $f_t=h_t\circ\phi_{\alpha_t}$, where $\alpha_t\in\Ac$. 
%Let $\h:=(h_1,\dots,h_T)\in\Hc^T$, $\bpsi:=(\bpsi_{1},\dots,\bpsi_{L})$ and $\bpsi_i:=(\psi_{i,1}\dots,\psi_{i,D_i})$, 
Let $\h=[h_1,\dots,h_T]^\top\in\Hc^T$, $\bal=[\alpha_1,\dots,\alpha_T]^\top\in\Ac^T$ and $\bpsi_i=[\psi_{i,1},\dots,\psi_{i,D_i}]^\top\in\Psi^{D_i},~\forall i\in[L]$. Hence, the problem is formulated as
\begin{align}
    \hat \h, \hat\bal, \{\hat{\bpsi}_{i}\}_{i=1}^L=&\underset{\underset{\{\bpsi_{i}\in\Psi_{i}^{D_i}\}_{i=1}^L}{\h\in\Hc^T,~\bal\in\Ac^T}}{\arg\min}\hat\Lc(\f)\label{formula:multipath}\\
    \text{where}~~~&\hat\Lc(\f)=\frac{1}{NT}\sum_{t=1}^T\sum_{i=1}^{N}\ell(h_t\circ\phi_{\alpha_t}(\x_{t,i}),y_{t,i}),\\
    &\phi_{\alpha_t}=\psi_{L,\alpha_t[L]}\circ\dots\circ\psi_{1,\alpha_t[1]}.
\end{align}
% \begin{align}
% \hat h_t, \hat\alpha_t, \hat{\psi}_{i,j}=\underset{\underset{\psi_{i,j}\in\Psi_{i,j}}{h_t\in\Hc,\alpha_t\in\Ac}}{\arg\min}\frac{1}{N}\sum_{t=1}^T\sum_{i=1}^{n_t}\ell(h_t\circ\phi_{{\alpha}_t}(\x_{t,i}),y_{t,i})~~\text{where}~~\phi_{\alpha_t}=\psi_{L,\alpha_t[L]}\circ\dots\circ\psi_{1,\alpha_t[1]}.\label{formula:multipath}
% \end{align}
Denoting $\bar\Dc=\frac{1}{T}\sum_{t\in[T]}\Dc_t$, we have that $\hat\Lc(\f)=\frac{1}{T}\sum_{t\in[T]}\hat\Lc_t(f_t)$ where $\hat\Lc_t(f_t)=\frac{1}{N}\sum_{i\in[N]}\ell(h_t\circ\phi_{\alpha_t}(\x_{t,i}),y_{t,i})$ and $\Lc(\f)=\E_{\bar\Dc}[\hat\Lc(\f)]$.

\red{
\begin{remark}
\end{remark}
}
